Evaluating Sensitivity to the Stick-Breaking Prior in Bayesian Nonparametrics

Bayesian models based on the Dirichlet process and other stick-breaking priors have been proposed as core ingredients for clustering, topic modeling, and other unsupervised learning tasks. However, due to the flexibility of these models, the consequences of prior choices can be opaque. And so prior specification can be relatively difficult. At the same time, prior choice can have a substantial effect on posterior inferences. Thus, considerations of robustness need to go hand in hand with nonparametric modeling. In the current paper, we tackle this challenge by exploiting the fact that variational Bayesian methods, in addition to having computational advantages in fitting complex nonparametric models, also yield sensitivities with respect to parametric and nonparametric aspects of Bayesian models. In particular, we demonstrate how to assess the sensitivity of conclusions to the choice of concentration parameter and stick-breaking distribution for inferences under Dirichlet process mixtures and related mixture models. We provide both theoretical and empirical support for our variational approach to Bayesian sensitivity analysis.

==> discussion.tex <==
Though the concept of local sensitivity in Bayesian nonparametric models is not
novel, the needed derivatives historically required for local sensitivity
required analytic derivations, which can be tedious to produce or perhaps
unavailable altogether. With the availability of modern automatic
differentiation tools, in combination with a variational approach to inference,
such difficulties are rendered obsolete. All that is necessary for computing
derivatives is the implementation in computer code of the $\mathrm{KL}$
objective as a function of variational parameters and the hyperparameter. Tools
such as \texttt{JAX}~\citep{jax2018github} provide the needed derivatives
exactly and automatically. We have shown that computing these derivatives and
linearizing the variational parameters can be an order of magnitude faster than
refitting the $\mathrm{KL}$ objective at a perturbed prior.

Computing the influence function---an expressive summary of all perturbations to
the prior ensity---is no more expensive than forming a single linear
approximation.  Though evaluating sensitivity to all possible perturbations is
impossible, we demonstrated how the influence function can guide our search for
functional perturbations that result in high sensitivity. The high-influence
perturbations can then be explored more closely either via our linear
approximation or by refitting.

Finally, we emphasize that concern about prior sensitivity is not unique to
Bayesian nonparametric models, and our local sensitivity framework also extends
to applications of variational inference to general Bayesian models. As our
examples show, non-robustness in posterior inferences may result in changes in
scientific conclusions, and our framework provides a fast, efficient way to
detect non-robustness in real applications.

